Orientations of Morse flow trees in Legendrian contact homology

Let $\Lambda$ be a closed, connected, spin Legendrian submanifold of the 1-jet space of a smooth $n$-dimensional manifold. We give a coherent orientation scheme for the moduli space of rigid Morse flow trees of $\Lambda$, implying that the Legendrian contact homology of $\Lambda$ with integer coefficients can be computed using Morse flow trees. If $n>1$ then this orientation scheme can be computed with an algorithm which uses intersections of oriented flow manifolds in $M$ together with combinatorial data coming from the trees.

==> introduction.tex <==
\section{Introduction}
Let $M$ be a smooth manifold of dimension $n$, and let $J^1(M)=T^*M \times \R$ denote its 1-jet
space, with  local coordinates $(x_1,\dotsc,x_n,y_1,\dotsc,y_n,z)$. This space can be given the structure  of a contact manifold, with contact distribution $\xi = \Ker ( dz- \sum_i y_i dx_i)$.   
 A submanifold $\Lambda \subset J^1(M)$ is called \emph{Legendrian} if it is $n$-dimensional and everywhere tangent to $\xi$, 
%and a \emph{Legendrian isotopy} is a continuous $1$-parameter family of Legendrian submanifolds. The \emph{Legendrian contact homology} of $\Lambda$ is a Legendrian isotopy invariant which was introduced by  Eliashberg, Givental and Hofer in \cite{sft}, and independently by Chekanov in \cite{chekanov} for the case $M=\R$. The analytical details underlying the theory were worked out by Ekholm, Etnyre and Sullivan in \cite{legsub, orientbok, pr}.
and a \emph{Legendrian isotopy} is a smooth $1$-parameter family of Legendrian submanifolds. The problem of classifying all Legendrian submanifolds of a contact manifold, up to Legendrian isotopy, is a central problem in contact geometry. This motivates finding  Legendrian invariants, that is, invariants that are preserved under Legendrian isotopies. One such invariant is \emph{Legendrian contact homology},  which is a homology theory that fits into the package of Symplectic Field Theory (SFT), introduced by Eliashberg, Givental and Hofer in the paper \cite{sft}. 

More recently, it has been shown that Legendrian contact homology can be used not only to study properties of Legendrian submanifolds, but also to compute symplectic invariants of Weinstein manifolds obtained by surgery along Legendrians. See e.g.\ ~\cite{surg2,surg1}. It has also been shown, for example in ~\cite{el,rm}, that this can be generalized and used for computations in homological mirror symmetry. This indicates the importance of being able to explicitly understand the Legendrian contact homology complex with integer coefficients. This paper should be an important step in that direction.   

% 
%  Legendrian contact homology was originally defined using pseudo-holomorphic curve techniques, but by the results of Ekholm in \cite{trees}, if the contact manifold is a 1-jet space one can instead use Morse theoretical arguments to compute the homology. We will use this latter setup to give an explicit algorithm to calculate the Legendrian contact homology for $\Lambda \subset J^1(M)$, with homology coefficients in $\Z$. This paper should be considered as a user's guide, and in particular no proofs will be given. Neither we will give a detailed introduction to Legendrian contact homology nor Morse flow trees. Instead we refer to \cite{orienttrees} for a complete exposition, both for definitions and for proofs.


Briefly, Legendrian contact homology is the homology of a differential graded algebra (DGA) associated to $\Lambda$.  One should note that Legendrian contact homology has not been worked out in full detail for all contact manifolds, but in the case when the contact manifold is given by  the 1-jet space $J^1(M) = T^*M \times \R $ of a manifold $M$, then the analytical details were established in \cite{pr}. In the special case $M = \R$, this was also done by Eliashberg in \cite{eliinv} and independently by Chekanov in \cite{chekanov}. 
%To handle the similar issues in the general setting of SFT,  the theory of Polyfolds developed by Hofer, Wysocki and Zehnder, see e.g.\ \cite{poly1}, and also  Pardon's work ~\cite{Pardon1, Pardon2} on virtual fundamental cycles, seem to be fruitful. 

In the case of a 1-jet space, the DGA of $\Lambda$ can be defined by considering the \emph{Lagrangian projection} 
$\Pi_\C: J^1(M) \to T^*M$. The generators of the algebra are then given by the double points of $\Pi_\C(\Lambda)$, which correspond to \emph{Reeb chords} of $\Lambda$. These are flow segments of the \emph{Reeb vector field}
 $\partial_z$, having start and end point on $\Lambda$.
The differential $\partial$ of the algebra counts certain rigid pseudo-holomorphic disks in $T^*M$ with boundary on $\Pi_\C(\Lambda)$. With a clever choice of almost complex structure on $T^*M$, one gets that the homology of this complex is a Legendrian invariant. 

If $M = \R$, then the count of pseudo-holomorphic disks reduces to combinatorics, as described by Chekanov in \cite{chekanov},  but in higher dimensions the Cauchy-Riemann equations give rise to non-linear partial differential equations, which are hard to solve. 
To simplify an analogous problem in Lagrangian Floer homology, Fukaya and Oh in \cite{fo} introduced \emph{gradient flow trees}, which are trees with edges along gradient flow lines in $M$, and gave a one-to-one correspondence between rigid gradient flow trees and rigid pseudo-holomorphic disks in $T^*M$ with boundary on the Lagrangians.
In \cite{trees}, Ekholm generalized this method to also work in the Legendrian contact homology setting. 



 In
the present paper we will combine the results in \cite{trees} with the results in \cite{orientbok}, where it is proved that Legendrian contact homology can be defined using $\Z$-coefficients, provided $\Lambda$ is spin. This corresponds to orienting moduli spaces of holomorphic disks in a coherent way and builds on the work of Fukaya, Oh, Ohta and Ono   in \cite{fooo}, where they describe a way to orient the determinant line of the $\dbar$-operator over the space of trivialized Lagrangian boundary conditions for the unit disk in $\C$. Since the differential in Legendrian contact homology counts rigid pseudo-holomorphic disks, the orientation of the moduli space at a disk $u$ corresponds to a sign of $u$. That the orientation of the moduli space is coherent means that all these signs cancels in $\partial^2$, so that we get $\partial^2 =0$.

The main result of this paper is the existence of a combinatorial algorithm for computing Legendrian contact homology with $\Z$-coefficients, using
orientations of  stable and unstable manifolds belonging to the Morse flow
trees of $\Lambda$. We refer to \cite{korta} for the explicit algorithm, in the present paper we focus on the analytical aspects of the proof that this algorithm indeed gives a coherent orientation scheme for moduli spaces of rigid Morse flow trees.  This is a generalization and an extension of the orientation scheme described in  \cite{kch} in the case when $\Lambda$ is the conormal lift of a knot in $\R^3$. 



\subsection{Outline}\label{sec:outline}
Let $\Lambda \subset J^1(M)$ be a spin Legendrian submanifold.
 We will assume that $\Lambda$ is \emph{front generic}, meaning that $\Pi:\Lambda \to M$ is an immersion outside a co-dimension 1 submanifold $\Sigma \subset \Lambda$. The points in $\Sigma$ we call \emph{cusp points}. We will also assume that $\Lambda$ has \emph{simple front singularities}, meaning that the points in $\Sigma$ are projected to standard cusp singularities under the front projection. See  \cite{trees}.  

 Locally, away from $\Sigma$, the Legendrian $\Lambda$ can be described as the multi-1-jet graph of locally defined functions $f_1,\dotsc,f_l: M \to \R$.
Fix a metric $g$ on $M$. The Morse flow trees of $\Lambda$ are defined using negative gradient flows of such function differences. I.e.\ the edges of the flow trees will be solution curves of $- \nabla (f_i-f_j)$ in $M$, and these curves are patched together at $2$- and $3$-valent vertices, where the local defining functions change. The tree is a directed graph with one root, and the direction of the edges are given by the flow direction of the defining vector fields. For example, at a $3$-valent vertex we can have an incoming flow line which solves $- \nabla(f_1-f_3)$, and two outgoing flow-lines solving $- \nabla (f_1-f_2)$ and $- \nabla (f_2 - f_3)$, respectively. See Figure \ref{fig:extree}. The $1$-valent vertices are either critical points of the flow lines ending at the vertex, or belong to $\Pi(\Sigma)$.  We give a more detailed description of flow trees in Section \ref{sec:tre}. 



\begin{figure}[ht]
\labellist
\small\hair 2pt
\pinlabel $\R$ [Br] at 101 320
\pinlabel ${f_1}$ [Br] at  456 285 
\pinlabel ${f_2}$ [Br] at 456 215
\pinlabel $f_3$ [Br] at 456 145
\pinlabel $\Gamma$ [Br] at 248 22
\pinlabel $M$ [Br] at 62 15
\endlabellist
\centering
\includegraphics[height=5cm, width=6.5cm]{fig/extree}
\caption{The local picture of a Morse flow tree $\Gamma$ in a neighborhood of a 3-valent vertex, given in the front projection. The graphs of the defining functions $f_1$, $f_2$ and $f_3$ are sketched, together with the lift of the tree to the sheets of $\Lambda$ determined by these functions. The shaded area indicates the corresponding $J$-holomorphic disk.}
\label{fig:extree}
\end{figure}

Each edge of the tree has two lifts to $\Lambda$, one for each of the sheets corresponding to the  defining functions of the edge. The 1-valent vertices which do not lift to $\Sigma$ will lift to end points of Reeb chords, and the Lagrangian projection of the lift of a tree will give a closed curve in $\Pi_\C(\Lambda)$. 

By the results in \cite{trees} there is a one-to-one correspondence between flow trees and pseudo-holomorphic disks defined by $\Lambda$. Briefly this works as follows. Consider the fiber scaling $s_\lambda:(x,y,z) \mapsto (x, \lambda y, \lambda z)$ which pushes $\Lambda$ towards the zero section. Then there is a choice of metric of $M$ and almost complex structure of $T^*M$, so that after a perturbation of $\Lambda$ there is a one-to-one correspondence between rigid flow trees of $\Lambda$ and sequences of $J$-holomorphic disks $u_\lambda$ in $T^*M$ with boundary on $\Pi_\C(s_\lambda(\Lambda))$. The disks are characterized by the property that their boundaries are arbitrarily close to the cotangent lift of the corresponding tree $\Gamma$. 
Moreover, the linearized boundary conditions of the disks tend to constant $\R^n$-boundary conditions, except at cusp points, where we get a split boundary condition which is constantly $\R$ in the first $n-1$ directions, and given by a uniform $\pm \pi$-rotation in the last direction, where the sign depends on the type of vertex. In addition, when we let $\lambda \to 0$, then  the domain of the disk will split up into a finite union of strips and strips with one slit.  See Section \ref{sec:slit}.       

The sign of a tree $\Gamma$ will be related to 
 orientations of the moduli spaces of pseudo-holomorphic disks $u_\lambda$, where the latter space will be given orientation by orienting the determinant lines of the linearized $\dbar$-operator at the disks. This orientation, in turn, is defined by using methods from \cite{fooo} and \cite{orientbok}, and is called the \emph{capping orientation} of $u_\lambda$. This orientation is related to choices of orientations of the stable and unstable manifolds of the critical points of the flow lines of $\Gamma$, and also to the chosen spin structure of $\Lambda$. 
For a definition of the capping orientation, see Section \ref{sec:background}.


Under the degeneration process, i.e.\ when $\lambda \to 0$, the rigid flow tree $\Gamma$ (or more precisely, the disks $u_\lambda$) splits up into \emph{elementary pieces}; pieces of the tree with at most $1$ vertex each. We use this to derive an algorithm for combinatorially calculating the capping orientation of  $\Gamma$ in the limit $\lambda =0$. Namely, we will give the elementary pieces of the tree orientations coming from the stable and unstable manifolds of the critical points contained in the tree. Then we glue the pieces back together again, and under this gluing we can understand the orientation of $\Gamma$ as oriented intersections of flow manifolds. Due to the rigidity of $\Gamma$, we will in the end get an oriented $0$-dimensional intersection, and by multiplying this by another sign calculated from combinatorial data from the tree, we obtain the capping orientation of the tree. 



The capping orientation of $u_\lambda$ and of $\Gamma$ will depend on several choices, which we call \emph{initial orientation choices} and which we describe in Section \ref{sec:orientconv}.
The main result is the following.

\begin{thm}\label{thm:mainthm}
Let $\Lambda \subset J^1(M)$ be a spin Legendrian submanifold, and assume that we have fixed all initial orientation choices. Then there is a coherent orientation scheme for the moduli space of rigid pseudo-holomorphic disks of $\Lambda$ so that the following holds.
Assume that $\Gamma$ is a rigid flow tree of $\Lambda$, and let
 $u_\lambda$, $\lambda \to 0$, be a sequence of rigid pseudo-holomorphic disks converging to  $\Gamma$ in the sense of \cite{trees}. Then there is a $\lambda_0>0$ so that the orientation of $u_\lambda$ is independent of $\lambda$ for $0 < \lambda<\lambda_0$, and this orientation can be computed in terms of intersections of oriented flow manifolds in $M$ together with combinatorial data coming from $\Gamma$. 
\end{thm}

For a complete statement of the algorithm for computing the orientation, we refer to \cite{korta}. Nevertheless, in Section \ref{sec:glupf} we indicate how all the formulas in \cite{korta} are derived. In particular, the reader will see what combinatorial data from the trees that are involved.

Theorem \ref{thm:mainthm} implies that the oriented 0-dimensional moduli spaces of flow trees are in one-to-one correspondence with the oriented $0$-dimensional moduli spaces of pseudo-holomorphic disks of $\Lambda$, and the orientation is preserved under the identification. This means, for example, that we can use flow trees to compute the Legendrian contact homology of $\Lambda$ with $\Z$-coefficients. This is one of the reasons why we give the tree $\Gamma$ the orientation from the corresponding pseudo-holomorphic disk. Namely, the 1-dimensional moduli spaces of pseudo-holomorphic disks have compactifications whose boundary consists of broken 0-dimensional disks. This helps us to prove that $\partial^2=0$, where $\partial$ is the differential in Legendrian contact homology. The corresponding compactification of spaces of Morse flow trees is more complicated.

\begin{rmk}
When calculating the differential $\partial$ in Legendrian contact homology, one has to compute an additional sign for the differential. Compare [\cite{orientbok}, Section 4.1] where the differential is defined as 
 \begin{equation}\label{eq:differentialen}
  \partial a  = \sum_{\dim \M_A(a;{\bf b})=0} (-1)^{(n-1)(|a|+1)} |\M_A(a;{\bf b})| A {\bf b}.
 \end{equation}
Here $|\M_A(a;{\bf b})|$ is the signed count of elements in the moduli space $\M_A(a;{\bf b})$ of rigid holomorphic disks, where the signs come from the capping orientations of the disks. The additional sign $(-1)^{(n-1)(|a|+1)} $ arises when we glue rigid disks together at the boundary of $1$-dimensional moduli spaces. 
\end{rmk}


\begin{rmk}
 The capping orientation of $u_\lambda$ defined in this paper will differ from the capping orientation defined in \cite{orientbok}. The reason for this is that the orientation in the present paper is easier to work with in the tree-setting, while the orientation in \cite{orientbok} is more efficient when, for example, proving invariance of the Legendrian contact homology under Legendrian isotopies. We refer to \cite{teckcob} for how these different choices affects the DGA. Also compare \cite{kch} where a similar issue is discussed. 
\end{rmk}





\subsection{Organization of the paper}
In Section \ref{sec:tre} we give an introduction to Morse flow trees, closely following \cite{trees}. In particular, we give a description of neighborhoods of partial flow trees, understood as submanifolds of $M$. It is these neighborhoods that we will use when calculating the orientation of $\Gamma$ from intersecting submanifolds in $M$.

% In Section \ref{sec:algen} we define the combinatorially algorithm which gives the sign $\sigma_\s(\Gamma)$, and in Section \ref{sec:examples} we give an elementary example of how this algorithm can be used.

In Section \ref{sec:background} we review some background materials and also define the capping orientation of a $J$-holomorphic disk. We use an approach similar to the one in \cite{orientbok}, but we will use slightly different orientation conventions. 

In Section \ref{sec:cutstab} we give a brief outline of how to associate a family of pseudo-\linebreak
holomorphic disks $u_\lambda$ to a rigid flow tree $\Gamma$, again following \cite{trees}. We also define the capping orientation of a flow tree $\Gamma$, which will be the capping  orientation of a sequence of pre-glued disks associated to the tree. Indeed, in \cite{trees} it is shown that for each $\lambda$  sufficiently small, there is a pre-glued disk $w_\lambda$ arbitrary close to $u_\lambda$ so that the boundary conditions induced by $w_\lambda$ are very easy to describe explicitly. 

In Section \ref{sec:glupf} we prove that the capping orientation of $\Gamma$ is independent of $\lambda$ for $\lambda$ sufficiently small, and that the capping orientation of $u_\lambda$ equals the capping orientation of $w_\lambda$ for such $\lambda$. This gives Theorem \ref{thm:mainthm}. The main technical results are proven in Section \ref{sec:stab} and Section \ref{sec:glupf}. In Appendix \ref{app:mini} we summarize some results concerning families of Fredholm operators. 




